Context Models for OOV Word Translation in Low-Resource Languages

Out-of-vocabulary word translation is a major problem for the translation of low-resource languages that suffer from a lack of parallel training data. This paper evaluates the contributions of target-language context models towards the translation of OOV words, specifically in those cases where OOV translations are derived from external knowledge sources, such as dictionaries. We develop both neural and non-neural context models and evaluate them within both phrase-based and self-attention based neural machine translation systems. Our results show that neural language models that integrate additional context beyond the current sentence are the most effective in disambiguating possible OOV word translations. We present an efficient second-pass lattice-rescoring method for wide-context neural language models and demonstrate performance improvements over state-of-the-art self-attention based neural MT systems in five out of six low-resource language pairs.

==> implementation.tex <==
\section{Data and Implementation}
\label{sec:implementation}
OOV word translation is studied on four low-resource languages, namely, Amharic, Uighur, Somali and Yoruba. The statistics about the data is tabulated in Table.\ref{tab:datastats}. 

\begin{table}
\begin{center}
	\begin{tabular}{| c | c | c | c | c |} \hline
    \#sent & \multirow{2}{*}{amh} & \multirow{2}{*}{uig} & \multirow{2}{*}{som} & \multirow{2}{*}{yor} \\ 
    (\#doc) & & & & \\ \hline
    \multirow{2}{*}{train} &63181 &99005 &52288 &41525 \\
    &(5941) &(18) &(8872) &(7538) \\ \hline
    \multirow{2}{*}{dev} &992 &686 &1054 &1060 \\
    &(158) &(3) &(252) &(228) \\ \hline
    \multirow{2}{*}{test} &511 &347 &552 &594 \\
    &(90) &(3) &(135) &(139) \\ \hline

    
%     \hline
%      \#sent/\#doc & train & dev & test  \\ \hline
%     amh & 63181/5941 & 992/158 & 511/90 \\ \hline
%     uig & 99005/18 & 686/3 & 347/3  \\ \hline
%     som & 52288/8872 & 1054/252 & 552/135 \\ \hline
%     yor & 41525/7538 & 1060/228 & 594/139 \\ \hline
    \end{tabular}
    \caption{Number of documents and sentences in the training, develop and test sets of the four low-resource languages.}
\end{center}
\label{tab:datastats}
\end{table}

\begin{table}
\label{tab:vocab}
\begin{center}
	\begin{tabular}{| c | c | c | c | c |} \hline
    & amh&uig&som&yor \\ \hline
    vocab &67330 &36914 &60039 &54519 \\ \hline
    oov in dev &2414 &892 &1497 &1287 \\ \hline
    oov in test &1071 &463 &760 &664 \\ \hline
    
%     \hline
%       & vocab & oov in dev & oov in test  \\ \hline
%     amh & 67330 & 2414 & 1071 \\ \hline
%     uig & 36914 & 892 & 463  \\ \hline
%     som & 60039 & 1497 & 760 \\ \hline
%     yor & 54519 & 1287 & 664 \\ \hline
    \end{tabular}
    \caption{The vocabulary sizes and number of OOV words in dev and test sets.}
\end{center}
\end{table}

Moses \cite{koehn2007moses} is used to implement phrase-based translation. Minimum error rate training \cite{bertoldi2009improved} is used to optimize for the weight vector $\omega$ (see Section \ref{phrase}). In preprocessing, sentences in training data are tokenized and true-cased. And sentences longer than 80 words are dropped in favor of memory usage in Moses decoding. Tokenization and true-casing are also done for the dev and test sets. 

In training, alignment is done under "grow-diag-final-and", reordering is done under "msd-bidirectional-fe" and trigram is used with kenLM \cite{heafield2011kenlm} for language modeling. The statistics about the vocabularies in the training sets and the OOV words in the dev and test sets after phrase-based translation is in Table.\ref{tab:vocab}. For comparison, a seq2seq model is trained using OpenNMT \cite{klein2017opennmt} on the training set upon the same preprocessing steps (results in Section \ref{sec:experiments}).

Related languages are used to help extract candidate translations for each OOV word. For example, a member of the Turkic language family as Uighur, the resource-richer Uzbek language serves as a proxy for extracting candidate translations for the OOV words in Uighur. Up to 50 candidates are extracted for each OOV work.

For OOV translation, several different methods are implemented. The key algorithm, document-contextual OOV translation is implemented in Dynet \cite{dynet}, where 2 LSTMs are stacked in the DCLMs, words are embedded in 16-dimension vectors, and the hidden representation is also of dimension 16. Long documents are partitioned into ones each with 4 sentences, for efficiency in training without losing much contextual dependency. For aDCLM, the attention layer dimension is 16. The complementary char-level neural language model has 2 layers, the input dimension is 16, and the dimension of the hidden representations is 16. 
The training data for DCLMs comes from WikiText-103's 29442 documents released in \cite{merity2016pointer} through data selection using Jaccard Index, which favors word presence over the word order in Moses hypotheses. Training references, dev hypotheses, and an extra lexicon of 20k common English words \footnote{\label{foo}\url{https://github.com/first20hours/google-10000-english}} are used in data selection. Training uses the dev reference from training the phrase-based model as the dev set.

For comparison, a 4-gram language model with a restricted vocabulary \cite{heafield2011kenlm} is trained on a combination of the training reference and a benchmark dataset \cite{41880} with sentence-level data selection based on the cross entropy \cite{moore2010intelligent} between the reference and the benchmark dataset under the 4-gram language model. A hypergraph decoding algorithm\footnote{\url{https://github.com/kpu/lazy}} for n-gram language models is used in lattice rescoring.

Based on \cite{roder2015exploring,woods2016exploiting}, PMI-based OOV translation is implemented, where the candidate word (phrases eliminated) that shares the highest PMI with the content words in the context is selected as the translation, and is added incrementally to the content word set. PMI statistics is computed over the WikiPedia dataset used in \cite{roder2015exploring}. The context window is allowed to straddle over sentences, paragraphs and documents, respectively.

Hypothetically, PageRank-based OOV translation overcomes the drawback of the PMI-based version that OOV words must be translated incrementally, but not jointly. In our PageRank implementation, for each sentence, translation candidates and content words in the context are nodes in a graph, where each candidate is connected with all content words, and content words are connected to each other. The weight on an edge is computed as the cosine similarity between the 300-dim GloVe embeddings \cite{pennington2014glove} of the two words being connected by the edge. For each OOV word, the candidate translation with the highest rank is selected as the translation upon PageRank convergence.


% One is often able to obtain reasonable translation results with much model tuning. Accordingly, statistical machine translation packages based on these approaches have been developed that can handle any language pairs. Among these packages Moses \cite{koehn2007moses}, OpenNMT \cite{klein2017opennmt}, Google seq2seq \cite{britz2017massive} and Nematus \cite{sennrich2017nematus} are the most representative. Specifically, Moses is based on log-linear models, supporting a variety of optimization objectives, hypotheses structures, optimization algorithms and evaluation measures \cite{neubig2016optimization}. The other three are based on seq2seq models with the attention mechanism, usually denoted as neural machine translation (NMT) models. 



==> tables.tex <==
\section{Tables}
\label{sec:tables}

\begin{table*}
\begin{center}
\begin{tabular}{| c | c | c | c | c | c |} \hline
\multicolumn{2}{|c|}{BLEU / UHR} & amh & uig & som & yor \\ \hline
\multirow{2}{*}{dev} &PBT 
&\textbf{16.22 / 48.8} &\textbf{13.35 / 45.3} &\textbf{24.91 / 58.5} &\textbf{19.68 / 51.5} \\\cline{2-6}
&NMT
&6.27 / 28.5 &6.81 / 34.9 &9.13 / 33.4 &6.15 / 31.3 \\ \hline
\multirow{2}{*}{test} &PBT 
&\textbf{16.74 / 48.8} &\textbf{7.83 / 41.9} &\textbf{23.27 / 57.2} &\textbf{18.26 / 50.2} \\\cline{2-6}
&NMT
&7.57 / 29.7 &4.64 / 31.6 &8.50 / 33.4 &6.25 / 32.3 \\ \hline
\end{tabular}
\caption{Baseline results in terms of BLEU and unigram hit rate (UHR) using phrase-based translation (PBT) and neural machine translation (NMT). Highlighted numbers show that phrase-based translation outperforms seq2seq on all datasets across all languages.}
\label{ccc}
\end{center}
\end{table*}


\begin{table*}
\begin{center}
\begin{tabular}{| c | c | c | c | c | c |} \hline
\multicolumn{2}{|c|}{BLEU / UHR} & amh & uig & som & yor \\ \hline
\multirow{2}{*}{dev} &(1) 
&16.27 / 48.9 &13.35 / 45.4 &24.86 / 58.5 &19.60 / 51.5 \\ \cline{2-6}
&(2)
&17.83 / 57.9 &17.30 / 64.5 &24.84 / 62.9 &20.06 / 55.1 \\ \hline
\multirow{2}{*}{test} &(1) 
&16.76 / 48.9 &7.92 / 43.1 &23.28 / 57.2 &18.14 / 50.1 \\ \cline{2-6}
&(2)
&18.14 / 50.1 &12.10 / 61.5 &23.76 / 61.6 &18.41 / 53.2 \\ \hline
\end{tabular}
\caption{Topline results in terms of BLEU and UHR obtained (1) by optimizing for BLEU+1 over all possible hypotheses, and (2) by aligning with reference.}
\end{center}
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{tabu}{| c | c | c | c | c |} \hline
BLEU / UHR & amh & uig & som & yor \\\hline
NMT&7.57 / 29.7 &4.64 / 31.6 &8.50 / 33.4 &6.25 / 32.3 \\\hline
PBMT&\textbf{16.74 / 48.8} &\textbf{7.83 / 41.9} &\textbf{23.27 / 57.2} &\textbf{18.26 / 50.2} \\\hline
\end{tabu}
\caption{BLEU scores and UHR (1) when candidate translations are extracted via related languages. (2) when candidate translations are extracted via related languages plus aligned words from reference. (3) when candidate translations are 20k common English words.}
\label{tab:res3}
\end{center}
\end{table*}

\begin{table*}[t]
\begin{center}
\begin{tabu}{| c | c |[2pt] c | c | c | c |} \hline
\multicolumn{2}{|c|[2pt]}{BLEU / UHR} & amh & uig & som & yor \\\tabucline[2pt]{-}
\multirow{1}{*}{baseline}
&PBMT 
&\textcolor{teal}{16.74 / 48.8} &\textcolor{teal}{7.83 / 41.9} &\textcolor{teal}{23.27 / 57.2} &\textcolor{teal}{18.26 / 50.2} \\\tabucline[2pt]{-}
topline-ref&align
&\textcolor{red}{18.14 / 50.1} &\textcolor{red}{12.10 / 61.5} &\textcolor{red}{23.76 / 61.6} &\textcolor{red}{18.41 / 53.2} \\\tabucline[2pt]{-}
% &PMI 
% &16.79 / 52.1 &16.39 / 60.2 &24.93 / 58.6 &19.98 / 53.0 \\\cline{2-6}
% \multirow{1}{*}{dev}&PageRank 
% &16.74 / 52.0 &16.63 / 63.0 &24.32 / 60.8 &19.77 / 53.9 \\\cline{2-6}
% \multirow{1}{*}{(2)}&4-gram 
% &17.35 / \textbf{55.6} &\textbf{16.97 / 63.5} &24.64 / \textbf{62.0} &19.83 / 54.2 \\\cline{2-6}
% &DCLM 
% &\textbf{17.37} / 55.5 &16.78 / 63.4 &\textbf{24.66} / 60.9 &\textbf{19.98 / 54.9} \\\tabucline[2pt]{-}
\multirow{5}{*}{topline-hyp+ref}&PMI 
&17.31 / 52.1 &9.70 / 53.2 &23.29 / 57.2 &\textcolor{violet}{18.46} / 51.2 \\\cline{2-6}
&PageRank 
&17.25 / 52.2 &9.79 / 55.0 &23.43 / 60.2 &18.16 / 52.4 \\\cline{2-6}
&4-gram 
&17.64 / 54.3 &\textcolor{violet}{10.87 / 58.3} &\textcolor{violet}{23.67 / 60.7} &18.25 / 52.5 \\\cline{2-6}
&RNNLM
&17.70 / 54.2 & 10.38 / 57.9 &23.46 / 60.5 &18.16 / 52.4 \\\cline{2-6}
&DCLM 
&\textcolor{violet}{17.81 / 54.8} &10.38 / 57.9 &23.55 / 60.6 &18.32 / \textcolor{violet}{52.8} \\\tabucline[2pt]{-}
%&PMI 
%&16.27 / 48.9 &13.35 / 45.3 &24.91 / 58.5 &19.68 / 51.5 \\\cline{2-6}
%\multirow{1}{*}{dev}&PageRank 
%&16.24 / 48.9 &13.35 / 45.3 &24.69 / 58.5 &19.60 / 51.4 \\\cline{2-6}
%\multirow{1}{*}{(1)}&4-gram 
%&16.26 / 49.0 &13.36 / 45.4 &24.80 / 58.4 &19.60 / 51.4 \\\cline{2-6}
%&DCLM 
%&\textbf{16.59 / 51.4} &\textbf{13.36 / 45.4} &\textbf{25.01 / 59.4} &\textbf{19.68 / 51.7} \\\tabucline[2pt]{-}
\multirow{5}{*}{hyp}&PMI 
&16.76 / 48.9 &7.87 / 42.1 &23.27 / 57.2 &18.26 / 50.2 \\\cline{2-6}
&PageRank 
&16.74 / 48.8 &7.86 / 42.2 &23.25 / 57.1 &18.20 / 50.2 \\\cline{2-6}
&4-gram 
&16.76 / 48.9 &7.87 / 42.3 &23.26 / 57.1 &18.21 / 50.2 \\\cline{2-6}
&RNNLM
&16.75 / 48.9 &8.54 / \textbf{47.4} &23.21 / 57.1 &18.29 / 50.7 \\\cline{2-6}
&DCLM 
&\textbf{16.76 / 49.0} &\textbf{8.57} / 46.9 &\textbf{23.27 / 57.3} &\textbf{18.30 / 50.6} \\\tabucline[2pt]{-}

% &PMI 
% &16.23 / 48.8 &13.35 / 45.3 &24.91 / 58.5 &19.63 / 51.5 \\\cline{2-6}
% \multirow{1}{*}{dev}&PageRank 
% &16.27 / 49.1 &13.38 / 45.7 &24.69 / 58.5 &19.58 / 51.2 \\\cline{2-6}
% \multirow{1}{*}{(3)}&4-gram 
% &16.37 / 49.8 &13.63 / 46.4 &24.47 / 58.9 &19.68 / 51.5 \\\cline{2-6}
% &DCLM 
% &\textbf{16.57 / 50.9} &\textbf{13.63 / 46.4} &\textbf{24.91 / 58.9} &\textbf{19.79 / 52.2} \\\tabucline[2pt]{-}
\multirow{5}{*}{common words}&PMI 
&16.74 / 48.8 &7.87 / 42.1 &23.26 / 57.2 &18.25 / 50.2 \\\cline{2-6}
&PageRank 
&16.75 / 48.9 &7.87 / 42.6 &23.25 / 57.1 &18.19 / 50.1 \\\cline{2-6}
&4-gram 
&16.84 / 49.6 &8.02 / 42.9 &23.27 / 57.2 &18.26 / 50.2 \\\cline{2-6}
&RNNLM
&17.07 / 50.7 &7.87 / 42.0 &23.20 / 57.1 &18.08 / 50.3 \\\cline{2-6}
&DCLM 
&\textbf{17.13 / 50.9} &\textbf{8.02 / 42.9} &\textbf{23.27 / 57.3} &\textbf{18.31 / 50.6} \\\hline
\end{tabu}
\caption{BLEU scores and UHR (1) when candidate translations are extracted via related languages. (2) when candidate translations are extracted via related languages plus aligned words from reference. (3) when candidate translations are 20k common English words.}
\label{tab:res1}
\end{center}
\end{table*}



\begin{table*}[t]
\begin{center}
\begin{tabu}{| c | c |[2pt] c | c | c | c |} \hline
\multicolumn{2}{|c|[2pt]}{BLEU / UHR} & amh & uig & som & yor \\\tabucline[2pt]{-}
\multirow{2}{*}{dev}&baseline 
&16.33 / 48.1 &34.81 / 63.3 &19.72 / 52.5 &19.39 / 51.8 \\\cline{2-6}
&rescoring 
&\textbf{17.02 / 49.9} &\textbf{35.36 / 63.7} &\textbf{19.73 / 52.5} &\textbf{20.62 / 54.1} \\\tabucline[2pt]{-}
\multirow{2}{*}{test}&baseline 
&15.15 / 46.7 &22.83 / 54.5 &18.33 / 51.8 &18.02 / 50.2 \\\cline{2-6}
&rescoring 
&\textbf{16.03 / 49.1} &22.79 / \textbf{54.6} &18.29 / \textbf{51.9} &\textbf{18.12 / 50.7} \\\hline
\end{tabu}
\caption{BLEU scores and UHR (1) when candidate translations are extracted via related languages. (2) when candidate translations are extracted via related languages plus aligned words from reference. (3) when candidate translations are 20k common English words.}
\label{tab:res2}
\end{center}
\end{table*}




\begin{table*}[t]
\begin{center}
\begin{tabu}{| c | c | c | c | c |} \hline
BLEU / UHR & amh & uig & som & yor \\\hline
baseline&16.74 / 48.8 &7.83 / 41.9 &23.27 / 57.2 &18.26 / 50.2 \\\hline
DCLM&17.12 / 50.8 &8.57 / 46.8 &23.27, 57.2 &18.28 / 50.3 \\\hline
DCLM+charLM&\textbf{17.13 / 50.9} &\textbf{8.57 / 46.9} &\textbf{23.27 / 57.3} &\textbf{18.31 / 50.6} \\\hline
\end{tabu}
\caption{BLEU scores and UHR (1) when candidate translations are extracted via related languages. (2) when candidate translations are extracted via related languages plus aligned words from reference. (3) when candidate translations are 20k common English words.}
\label{tab:res3}
\end{center}
\end{table*}
